New Textual Corpora for Serbian Language Modeling

This paper will present textual corpora for Serbian (and Serbo-Croatian), usable for the training of large language models and publicly available at one of the several notable online repositories. Each corpus will be classified using multiple methods and its characteristics will be detailed. Additionally, the paper will introduce three new corpora: a new umbrella web corpus of Serbo-Croatian, a new high-quality corpus based on the doctoral dissertations stored within National Repository of Doctoral Dissertations from all Universities in Serbia, and a parallel corpus of abstract translation from the same source. The uniqueness of both old and new corpora will be accessed via frequency-based stylometric methods, and the results will be briefly discussed.

==> settings/right/settings.tex <==
% ----------- update from the preamble % -------------

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{indentfirst}

\usepackage{lmodern}

\usepackage[english]{babel}
\usepackage{csquotes}

\usepackage{amsmath}
\usepackage[authordate,backend=biber,dashed=false]{biblatex-chicago}

%
% ------------ biblioteke ----------
%
% specificne dimenzije stranica
\usepackage{geometry}
 \geometry{
	top=23mm,
	bottom=21mm,
	left=12mm,
	right=20mm
 }
% slike
\usepackage{graphicx}
% putanja do direktorijuma sa slikama
\graphicspath{ {images/} }
% proizvoljne boje
\usepackage[dvipsnames]{xcolor}
% poravnanje teksta
\usepackage{ragged2e}
% dupla linija u tabeli
\usepackage{array}
% zbog adjustwidth svojstva
\usepackage{changepage}
% podesavanje zaglavlja
\usepackage{fancyhdr}
% definicija okruzenja koje koristi parbox-ove
%% ne moze klasican nacin jer ne dozvoljava nebalansirane zagrade
\usepackage{environ}
% linkovi
\usepackage[colorlinks = true,
            linkcolor = Sepia,
            urlcolor  = Mahogany,
            citecolor = BrickRed,
            anchorcolor = Sepia]{hyperref}
% fusnote
\usepackage{footnote}
\makesavenoteenv{tabular} %% fusnote "znaju" da ne rade u tabelama
% bibliografija



%
% ------------ podesavanje fonta ----------
%
%\renewcommand\familydefault{\sfdefault} %% deluje neozbiljno

% debljina linije zaglavlja
\renewcommand{\headrulewidth}{0.4pt}

%
% ----------------- boje -------------------------
%
\definecolor{light_gray}{rgb}{0.5, 0.5, 0.5}
\definecolor{dark_gray}{rgb}{0.4, 0.4, 0.4}
\definecolor{darker_gray}{rgb}{0.2, 0.2, 0.2}

%
% ----------------- definicije novih naredbi ---------------
%
% 

%%%%% UDC %%%%%%%%
\newcommand{\udc}[1]{\begin{adjustwidth}{-0.5cm}{}{\par\textcolor{dark_gray}{\parbox{\textwidth}{\begin{flushright}\texttt{UDC #1}\end{flushright}}}}\end{adjustwidth}}
%%%%% DOI %%%%%%%%
\newcommand{\ddoi}[1]{\begin{adjustwidth}{-0.5cm}{}{\par\textcolor{dark_gray}{\parbox{\textwidth}{\begin{flushright}\texttt{DOI #1}\end{flushright}}}}\end{adjustwidth}}

% autor
\renewcommand{\author}[1]{\hfill #1 \newline}
% institution
\newcommand{\institution}[1]{
	\textcolor{darker_gray}{\textit{\small \hfill #1}} \newline
}
% email
\renewcommand{\email}[1]{\textcolor{light_gray}{\hfill \small #1} \newline}

%
% ----------------- redefinicije postojecih naredbi ---------------
%
% naslov
\renewcommand{\title}[1]{\begin{center}\Large\bfseries\boldmath#1\end{center}}


%
% ----------------- definicija novih okruzenja ---------------
%
% okruzenje za glavni deo = apstrakt, datumi, autori, prevod (sve)
\newenvironment{main}
		{\begin{adjustwidth}{-0.2cm}{}\begin{tabular}{ l @{~} @{~} !{\vrule width 2pt}| @{~} l }}
		{\end{tabular}\end{adjustwidth}}
% okruzenje za apstrakt
\NewEnviron{abstractenv}{%
	 %\vspace{-1cm}  %% fix zbog margina apstrakta
		%  sazetak  
		\parbox[t]{0.6\textwidth}{	
			\begin{adjustwidth}{-1cm}{}	
				\begin{abstract}							
					% tekst sazetka
					\BODY						
				\end{abstract}
			\end{adjustwidth}
		}
}% 
% podaci o autorima
\NewEnviron{authorsenv}{%
  \parbox[t]{0.4\textwidth}{%
      \BODY
   }
}%   

%%%%% dodaci 2021.

\usepackage{hyperref}
\usepackage{comment}
